Ultramassive black holes formed by triple quasar mergers at $z\sim 2$

The origin of rare and elusive ultramassive black holes (UMBH, with MBH > 1e10 Msun) is an open question. Using the large volume cosmological hydrodynamic simulation ASTRID, we report on the formation of an extremely massive UMBH with MBH ~ 1e11 Msun at z~2. The UMBH is assembled as a result of two successive mergers of massive galaxies each with stellar mass M* > 3e11 Msun that also produces a bright, rare triple quasar system powered by three ~10^9 Msun black holes. The second merger of supermassive black holes (SMBHs) follows the first after 150 Myrs. The merger events lead to sustained Eddington accretion onto the central SMBH, forming an UMBH in the center of a massive compact stellar core with M* > 2e12 Msun. The strong feedback of the UMBH quenches the surrounding star formation to < 10 Msun/yr in the inner 50 kpc/h region. There are two more UMBHs with MBH > 5e10 Msun at z>2 in ASTRID which are also produced by major mergers of galaxies, and their progenitors can be observed as quasar triplets of lower luminosity. The rarely observed quasar multiples can be the cradle of UMBHs at high redshift, and likely end up in the center of the most massive clusters.

==> Sec2_Method_old.tex <==
\section{Simulation}
\label{section2:Method}

\astrid is a cosmological hydrodynamical simulation performed using a new version of the \texttt{MP-Gadget} simulation code. 
\texttt{MP-Gadget} is optimized to run on the massively parallel high performance computer systems with high scalability and carry out missions of large cosmological simulations.

\astrid contains $5500^3$ cold dark matter (DM) particles in a $250 \hmpc$ side box, and an initially equal number of SPH hydrodynamic mass elements.
The cosmological parameters used in \astrid are from \citep{Planck}, with $\Omega_0=0.3089$, $\Omega_\Lambda=0.6911$, $\Omega_{\rm b}=0.0486$, $\sigma_8=0.82$, $h=0.6774$, $A_s = 2.142 \times 10^{-9}$, $n_s=0.9667$. 
The gravitational softening length is $\epsilon_{\rm g} = 1.5 \hkpc$ for both DM and gas particles.
\astrid achieves a dark matter particle mass resolution of $9.6\times 10^6 \msun$ and $M_{\rm gas} = 1.3 \times 10^6 \hmsun$ in the initial conditions.


\astrid implements a variety of sub-grid models for physics governing the formation of galaxies and SMBHs and their associated supernova and AGN feedback, inhomogeneous hydrogen and helium reionization, and the effect of massive neutrinos.
Here we briefly summarize the physical models used in the simulation and refer the readers to the introductory paper \cite{Ni-Asterix,Bird-Asterix} for more detailed descriptions.
 
In \astrid, gas is allowed to cool via primordial radiative cooling \cite{Katz1996ApJS..105...19K} and via metal line cooling, with the gas and stellar metallicities traced following \cite{Vogelsberger:2014}.
Patchy reionization of hydrogen is performed with a spatially varying ultra-violet background using a semi-analytic method based on radiative transfer simulations \citep{Battaglia2013ApJ...776...81B}. 
For the ionized regions, we applied the ionizing ultra-violet background from \cite{FG2020} and gas self-shielding following \cite{Rahmati:2013}. 
Star formation is implemented based on the multi-phase star formation model in \cite{SH03}, and account for the effects of molecular hydrogen~\citep{Krumholz2011ApJ...729...36K}.
Type II supernova wind feedback is included following \cite{Okamoto2010}, assuming wind speeds proportional to the local one dimensional dark matter velocity dispersion.


Subgrid models for SMBH applied in \astrid can be summarized as follows.
SMBHs are represented by particles which can accrete gas, merge with each other and apply feedback to their baryonic surroundings.
We use halo-based seeding where the BHs are seeded in haloes with \{ $M_{\rm halo,FOF} > 5 \times 10^9 \hmsun$; $M_{\rm *,FOF} >2 \times 10^6 \hmsun$\}. 
Seed masses are stochastically drawn from a power law probability distribution, with a mass between $3\times10^{4} \hmsun$ and $3\times10^{5} \hmsun$ and power law index $n = -1$.
The gas accretion rate onto the BH is estimated via the Bondi-Hoyle-Lyttleton-like prescription \citep{DSH2005}.
We allow for short periods of super-Eddington accretion in the simulation, but limit the accretion rate to $2$ times the Eddington accretion rate.
The BH radiates with a bolometric luminosity $L_{\rm bol}$ proportional to the accretion rate $\dot{M}_{\rm BH}$, with a mass-to-light conversion efficiency $\eta=0.1$ in an accretion disk according to \cite{Shakura1973}.
5\% of the radiated energy is coupled to the surrounding gas as the AGN feedback.
The feedback from SMBHs includes what is often referred to as a quasar-mode or thermal feedback as well as the kinetic feedback.
\yueying{How do we talk about kinetic feedback here?}
Dynamics of the SMBHs is modelled with a newly developed (sub-grid) dynamical friction \citep{Tremmel2015,Chen2021} to replace the original implementation that directly repositioned the BHs to the local minimum potential.
This model gives well-defined BH trajectories and velocities and therefore provides a more physical treatment of the mergers of SMBHs.
Two BHs can be merged if their separation is within two times the spatial resolution $2\epsilon_g$, once their kinetic energy is dissipated by dynamical friction and they are gravitationally bound to each other.
The validation of the dynamical friction model in cosmological simulations was performed in \cite{Chen2021}.

% In \astrid, evolution of BHs are logged with high time-resolution to a separate catalogue, allowing us to follow the detailed growth history of BHs in the simulation, build the merger trees of BHs and trace the trajectory of BH merger events down to $\kpc$ scale.  


Currently, the \astrid simulation has reached $z=2$. 
It is the largest cosmological simulation of galaxy formation to date that covers the epoch of cosmic noon, where both star formation and quasars reach their peak activity.
It contains $5 \times 10^{5}$ halos with a FOF mass greater than $10^{12} \msun$ and $2 \times 10^{3}$ halos with a mass greater than $10^{13} \msun$.
Galaxies in the simulation are identified through \texttt{SUBFIND} \citep{2001MNRAS.328..726S} in a post-processed manner. 
At $z=2$, \astrid contains a statistical sample of very massive galaxies and bright quasars, with about $3 \times 10^{3}$ galaxies with $\mstar>10^{11} \msun$ and 13 galaxies with $\mstar \geq 10^{12} \msun$. 
It produces 709 BHs with $\mbh > 10^{9} \msun$, three out of which have $\mbh > 5 \times 10^{10} \msun$ and the most massive one has reached $10^{11} \msun$. 
The large volume of \astrid provides us with an ideal tool to study the galaxy and quasar population at cosmic noon.


